Towards Transitive-free Digraphs

In a digraph $D$, an arc $e=(x,y) $ in $D$ is considered transitive if there is a path from $x$ to $y$ in $D- e$. A digraph is transitive-free if it does not contain any transitive arc. In the Transitive-free Vertex Deletion (TVD) problem, the goal is to find at most $k$ vertices $S$ such that $D-S$ has no transitive arcs. In our work, we study a more general version of the TVD problem, denoted by $\ell$-Relaxed Transitive-free Vertex Deletion ($\ell$-RTVD), where we look for at most $k$ vertices $S$ such that $D-S$ has no more than $\ell$ transitive arcs. We explore $\ell$-RTVD on various well-known graph classes of digraphs such as directed acyclic graphs (DAGs), planar DAGs, $\alpha$-bounded digraphs, tournaments, and their multiple generalizations such as in-tournaments, out-tournaments, local tournaments, acyclic local tournaments, and obtain the following results. Although the problem admits polynomial-time algorithms in tournaments, $\alpha$-bounded digraphs, and acyclic local tournaments for fixed values of $\ell$, it remains NP-hard even in planar DAGs with maximum degree 6. In the parameterized realm, for $\ell$-RTVD on in-tournaments and out-tournaments, we obtain polynomial kernels parameterized by $k+\ell$ for bounded independence number. But the problem remains fixed-parameter intractable on DAGs when parameterized by $k$.

==> abstract.tex <==
\begin{abstract}
	In a digraph $D$, an arc $e=(x,y) $ in $D$ is considered transitive if there is a path from $x$ to $y$ in $D- e$. A digraph is transitive-free if it does not contain any transitive arc. In the {\sc Transitive-free Vertex Deletion} (TVD) problem, the goal is to find at most $k$ vertices $S$ such that $D-S$ has no transitive arcs. In our work, we study a more general version of the TVD problem, denoted by {\sc $\ell$-RTVD}, where we look for at most $k$ vertices $S$ such that $D-S$ has no more than  $\ell$ transitive arcs. We explore {\sc $\ell$-RTVD} on various well-known graph classes of digraphs such as directed acyclic graphs (DAGs), planar DAGs, $\alpha$-bounded digraphs, tournaments, and their multiple generalizations such as in-tournaments, out-tournaments, local tournaments, local acyclic tournaments and obtain the following results. While the problem admits polynomial-time algorithms in tournaments, $\alpha$-bounded digraphs, and acyclic local tournaments for fixed values of $\ell$, it remains $\textsf{NP}$-Hard even in planar DAGs with maximum degree 6.	In the parameterized realm, for {\sc $\ell$-RTVD} on in-tournaments and out-tournaments, we obtain polynomial kernels parameterized by $k+\ell$ for bounded independence number. But the problem remains fixed-parameter intractable on DAGs when parameterized by $k$.
	
	\end{abstract}
%

==> local_tour.tex <==


\section{A linear kernel for \lvd on local tournaments}

\begin{theorem}
\lvd on local tournaments admits a kernel with $O(\ell+k)$ vertices.
\end{theorem}

Let $(D,k,\ell)$ be an instance of \lvd on the local tournament.
